Modeling Human Driving Behavior through Generative Adversarial Imitation Learning

An open problem in autonomous vehicle safety validation is building reliable models of human driving behavior in simulation. This work presents an approach to learn neural driving policies from real world driving demonstration data. We model human driving as a sequential decision making problem that is characterized by non-linearity and stochasticity, and unknown underlying cost functions. Imitation learning is an approach for generating intelligent behavior when the cost function is unknown or difficult to specify. Building upon work in inverse reinforcement learning (IRL), Generative Adversarial Imitation Learning (GAIL) aims to provide effective imitation even for problems with large or continuous state and action spaces, such as modeling human driving. This article describes the use of GAIL for learning-based driver modeling. Because driver modeling is inherently a multi-agent problem, where the interaction between agents needs to be modeled, this paper describes a parameter-sharing extension of GAIL called PS-GAIL to tackle multi-agent driver modeling. In addition, GAIL is domain agnostic, making it difficult to encode specific knowledge relevant to driving in the learning process. This paper describes Reward Augmented Imitation Learning (RAIL), which modifies the reward signal to provide domain-specific knowledge to the agent. Finally, human demonstrations are dependent upon latent factors that may not be captured by GAIL. This paper describes Burn-InfoGAIL, which allows for disentanglement of latent variability in demonstrations. Imitation learning experiments are performed using NGSIM, a real-world highway driving dataset. Experiments show that these modifications to GAIL can successfully model highway driving behavior, accurately replicating human demonstrations and generating realistic, emergent behavior in the traffic flow arising from the interaction between driving agents.

==> macros.tex <==
\usepackage{cleveref}
% \usepackage{algorithm}
% \usepackage{algorithmicx}
% \usepackage[noend]{algpseudocode}
\usepackage{acronym}
%\usepackage{color,xcolor}
\usepackage{verbatim}
\usepackage{booktabs}
\usepackage{siunitx}
\usepackage{graphicx,caption}
\usepackage{amsmath,amssymb,stmaryrd,mathtools}
\usepackage[keeplastbox]{flushend}
\usepackage{graphics}
% \usepackage{subcaption}
\usepackage{suffix}
\usepackage{xstring}
\usepackage{xparse}
\usepackage{expl3}

\usepackage{wrapfig}
\usepackage{amsmath}
\usepackage{tikz}
\usetikzlibrary{arrows,backgrounds,calc}
\usepackage{relsize}

%% PGF preamble
\RequirePackage{luatex85}
% \documentclass[tikz]{standalone}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\pgfplotsset{every axis legend/.append style={%
		cells={anchor=west}}
}
\usepgfplotslibrary{polar}
\usetikzlibrary{arrows}
\tikzset{>=stealth'}

\definecolor{C1}{rgb}{0.0, 0.447, 0.741}
\definecolor{C1_light}{rgb}{0.0, 0.6032388663967612, 1.0}
\definecolor{C2}{rgb}{0.85, 0.325, 0.098}
\definecolor{C3}{rgb}{0.929, 0.694, 0.125}
\definecolor{C4}{rgb}{0.494, 0.184, 0.556}
\definecolor{C5}{rgb}{0.466, 0.674, 0.188}
\definecolor{C6}{rgb}{0.301, 0.745, 0.933}
\definecolor{C7}{rgb}{0.635, 0.078, 0.184}

\usepgfplotslibrary{groupplots}

\usetikzlibrary{shapes.geometric, arrows}

\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=2cm, minimum height=1cm,text centered, draw=black, fill=none]
\tikzstyle{arrow} = [thick,->,>=stealth]

%% \usepackage[letterpaper, portrait, margin=1in]{geometry}
%
%% *** CITATION PACKAGES ***
%% \usepackage{cite}
%% *** ALIGNMENT PACKAGES ***
%\usepackage{array}
%% The following packages can be found on http:\\www.ctan.org
%\usepackage{graphics} % for pdf, bitmapped graphics files
%%\usepackage{epsfig} % for postscript graphics files
%%\usepackage{mathptmx} % assumes new font selection scheme installed
%%\usepackage{times} % assumes new font selection scheme installed
%% \usepackage{bbold}
%% \usepackage{subfig}
%\usepackage{subcaption}
%\usepackage{multirow}
%
%%%
%\usepackage{suffix}
%\usepackage{xstring}
%\usepackage{xparse}
%\usepackage{expl3}
%
%
%%\PassOptionsToPackage{hyphens}{url}
%%\usepackage[options]{nohyperref}
%\usepackage{url}
%\usepackage{dsfont}
%%\usepackage[]{algorithm2e}
%\usepackage{algorithm}
%\usepackage{algorithmicx}
%\usepackage[noend]{algpseudocode}
%\usepackage{hyperref}
%\usepackage{cleveref}
%\usepackage{acronym}
%\usepackage{color,xcolor}
%\usepackage{verbatim}
%\usepackage{booktabs}
%\usepackage{siunitx}
%\usepackage{graphicx,caption}
%\usepackage{amsmath,amssymb,stmaryrd,mathtools}
%\usepackage[keeplastbox]{flushend}
%\usepackage{algorithm}
%%\usepackage[noend]{algpseudocode}
%\usepackage{cite}
%\usepackage{hyperref}
%\usepackage{cleveref}
%\usepackage{acronym}
%\usepackage{color,xcolor}
%\usepackage{verbatim}
%\usepackage{booktabs}
%\usepackage{siunitx}
%% correct bad hyphenation here
%\hyphenation{op-tical net-works semi-conduc-tor}
%%\usepackage{subcaption}
%
%
%\newcommand{\norm}[1]{\left\lVert #1 \right\rVert} % http://tex.stackexchange.com/questions/70020/how-to-write-euclidean-distance
%\newcommand{\abs}[1]{\left\lvert #1 \right\rvert} % http://tex.stackexchange.com/questions/70020/how-to-write-euclidean-distance
%
%\graphicspath{{./figures/}}
%
%%argmin
%\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\ignore}[1]{}
%%\newcommand{\comment}[1]{{\color{red} #1 }}
%\newtheorem{definition}{Definition}[section]
%\newtheorem{theorem}{Theorem}[section]
%%\newtheorem{proof}{Proof}[section]
%
%
%\newcommand{\eg}{e.\,g.,\ }
%\newcommand{\ie}{i.\,e.,\ }
%\newcommand{\etal}{{et~al.}}
%
%%introduce \powerset - hint by http://matheplanet.com/matheplanet/nuke/html/viewtopic.php?topic=136492&post_id=997377
%\DeclareFontFamily{U}{MnSymbolC}{}
%\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}
%\DeclareFontShape{U}{MnSymbolC}{m}{n}{
%    <-6>  MnSymbolC5
%   <6-7>  MnSymbolC6
%   <7-8>  MnSymbolC7
%   <8-9>  MnSymbolC8
%   <9-10> MnSymbolC9
%  <10-12> MnSymbolC10
%  <12->   MnSymbolC12%
%}{}
%\DeclareMathSymbol{\powerset}{\mathord}{MnSyC}{180}
%\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
%
%\definecolor{orange}{rgb}{1, .36, .08}
%\definecolor{darkmagenta}{rgb}{0.698,0,0.698}
%\newcommand{\dorsa}[1]{\normalsize{\color{darkmagenta}(DS:\ #1)}}
%
%%%% Vijay's edits %%%
%\definecolor{vg_edit_color}{rgb}{0, 0.0, 1.0}
%\newcommand{\vg}[1]{\normalsize{\color{vg_edit_color} VG:\ #1}}
%%%%%%%%%%%%%%%%%%%%%%
%
%% optimization commands
%\newcommand{\M}[1]{\underset{#1}{\text{minimize}}\;}
%\newcommand{\AM}[1]{\underset{#1}{\text{argmin}}\;}
%\newcommand{\ST}{\text{subject to}}
%

\newcommand{\eg}{e.\,g.,\ }
\newcommand{\ie}{i.\,e.,\ }
\newcommand{\etal}{{et~al.}}
\usepackage{cleveref}
% \newcommand{\citet}[1]{\citeauthor{#1}~\shortcite{#1}}

% this package is for todo notes!
%===todonotes====
% \usepackage{todonotes}
\usepackage{soul}
\definecolor{smoothgreen}{rgb}{0.7,1,0.7}
\sethlcolor{smoothgreen}

\newcommand{\todopara}[1]{\vspace{0px} %
\todo[inline, color=black!10]{\textbf{[Paragraph:]} {#1}} %
}
\newcommand{\todonote}[1]{\vspace{0px} %
\todo[inline, color=green!30]{\textbf{[Note:]} {#1}} %
}
\newcommand{\todoQ}[1]{\vspace{0px} %
\todo[inline, color=orange!50]{\textbf{[Note:]} {#1}} %
}
\newcommand{\todohere}[1]{\hl{(\textbf{TODO:} #1)}}

\newcommand{\hidetodos}{
\renewcommand{\todopara}[1]{}
\renewcommand{\todonote}[1]{}
\renewcommand{\todoQ}[1]{}
\renewcommand{\todohere}[1]{}}
%\hidetodos
%===end todonotes===
%
%%% PGF preamble
%\RequirePackage{luatex85}
%% \documentclass[tikz]{standalone}
%\usepackage{pgfplots}
%\pgfplotsset{compat=newest}
%\pgfplotsset{every axis legend/.append style={%
%cells={anchor=west}}
%}
%\usepgfplotslibrary{polar}
%\usetikzlibrary{arrows}
%\tikzset{>=stealth'}
%
%\definecolor{C1}{rgb}{0.0, 0.447, 0.741}
%\definecolor{C1_light}{rgb}{0.0, 0.6032388663967612, 1.0}
%\definecolor{C2}{rgb}{0.85, 0.325, 0.098}
%\definecolor{C3}{rgb}{0.929, 0.694, 0.125}
%\definecolor{C4}{rgb}{0.494, 0.184, 0.556}
%\definecolor{C5}{rgb}{0.466, 0.674, 0.188}
%\definecolor{C6}{rgb}{0.301, 0.745, 0.933}
%\definecolor{C7}{rgb}{0.635, 0.078, 0.184}
%
%\usepgfplotslibrary{groupplots}
%
%\usetikzlibrary{shapes.geometric, arrows}
%
%\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=2cm, minimum height=1cm,text centered, draw=black, fill=none]
%\tikzstyle{arrow} = [thick,->,>=stealth]
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "root"
%%%% End:
%% *** FLOAT PACKAGES ***
%%
%%\usepackage{fixltx2e}
%% fixltx2e, the successor to the earlier fix2col.sty, was written by
%% Frank Mittelbach and David Carlisle. This package corrects a few problems
%% in the LaTeX2e kernel, the most notable of which is that in current
%% LaTeX2e releases, the ordering of single and double column floats is not
%% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
%% single column figure to be placed prior to an earlier double column
%% figure.
%% Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
%% corrections already built into the system in which case a warning will
%% be issued if an attempt is made to load fixltx2e.sty as it is no longer
%% needed.
%% The latest version and documentation can be found at:
%% http://www.ctan.org/pkg/fixltx2e
%
%
%%\usepackage{stfloats}
%% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
%% the ability to do double column floats at the bottom of the page as well
%% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
%% LaTeX2e). It also provides a command:
%%\fnbelowfloat
%% to enable the placement of footnotes below bottom floats (the standard
%% LaTeX2e kernel puts them above bottom floats). This is an invasive package
%% which rewrites many portions of the LaTeX2e float routines. It may not work
%% with other packages that modify the LaTeX2e float routines. The latest
%% version and documentation can be obtained at:
%% http://www.ctan.org/pkg/stfloats
%% Do not use the stfloats baselinefloat ability as the IEEE does not allow
%% \baselineskip to stretch. Authors submitting work to the IEEE should note
%% that the IEEE rarely uses double column equations and that authors should try
%% to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
%% packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
%% such ways.
%% Do not attempt to use stfloats with fixltx2e as they are incompatible.
%% Instead, use Morten Hogholm'a dblfloatfix which combines the features
%% of both fixltx2e and stfloats:
%%
%% \usepackage{dblfloatfix}
%% The latest version can be found at:
%% http://www.ctan.org/pkg/dblfloatfix
%
%%\ifCLASSOPTIONcaptionsoff
%%  \usepackage[nomarkers]{endfloat}
%% \let\MYoriglatexcaption\caption
%% \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
%%\fi
%% endfloat.sty was written by James Darrell McCauley, Jeff Goldberg and 
%% Axel Sommerfeldt. This package may be useful when used in conjunction with 
%% IEEEtran.cls'  captionsoff option. Some IEEE journals/societies require that
%% submissions have lists of figures/tables at the end of the paper and that
%% figures/tables without any captions are placed on a page by themselves at
%% the end of the document. If needed, the draftcls IEEEtran class option or
%% \CLASSINPUTbaselinestretch interface can be used to increase the line
%% spacing as well. Be sure and use the nomarkers option of endfloat to
%% prevent endfloat from "marking" where the figures would have been placed
%% in the text. The two hack lines of code above are a slight modification of
%% that suggested by in the endfloat docs (section 8.4.1) to ensure that
%% the full captions always appear in the list of figures/tables - even if
%% the user used the short optional argument of \caption[]{}.
%% IEEE papers do not typically make use of \caption[]'s optional argument,
%% so this should not be an issue. A similar trick can be used to disable
%% captions of packages such as subfig.sty that lack options to turn off
%% the subcaptions:
%% For subfig.sty:
%% \let\MYorigsubfloat\subfloat
%% \renewcommand{\subfloat}[2][\relax]{\MYorigsubfloat[]{#2}}
%% However, the above trick will not work if both optional arguments of
%% the \subfloat command are used. Furthermore, there needs to be a
%% description of each subfigure *somewhere* and endfloat does not add
%% subfigure captions to its list of figures. Thus, the best approach is to
%% avoid the use of subfigure captions (many IEEE journals avoid them anyway)
%% and instead reference/explain all the subfigures within the main caption.
%% The latest version of endfloat.sty and its documentation can obtained at:
%% http://www.ctan.org/pkg/endfloat
%%
%% The IEEEtran \ifCLASSOPTIONcaptionsoff conditional can also be used
%% later in the document, say, to conditionally put the References on a 
%% page by themselves.
%
%
%

